Real-time Tracking in a Status Update System with an Imperfect Feedback Channel

We consider a status update system consisting of a finite-state Markov source, an energy-harvesting-enabled transmitter, and a sink. The forward and feedback channels between the transmitter and the sink are error-prone. We study the problem of minimizing the long-term time average of a (generic) distortion function subject to an energy causality constraint. Since the feedback channel is error-prone, the transmitter has only partial knowledge about the transmission results and, consequently, about the estimate of the source state at the sink. Therefore, we model the problem as a partially observable Markov decision process (POMDP), which is then cast as a belief-MDP problem. The infinite belief space makes solving the belief-MDP difficult. Thus, by exploiting a specific property of the belief evolution, we truncate the state space and formulate a finite-state MDP problem, which is then solved using the relative value iteration algorithm (RVIA). Furthermore, we propose a low-complexity transmission policy in which the belief-MDP problem is transformed into a sequence of per-slot optimization problems. Simulation results show the effectiveness of the proposed policies and their superiority compared to a baseline policy. Moreover, we numerically show that the proposed policies have switching-type structures.

==> structur.tex <==
% In the following theorem shows that the $\lambda$-optimal policy has a switching-type structure for decision making respect to the age of the packets in the system.
% \theorem{Any $\lambda$-optimal policy of problem \eqref{mdp1} has a switching-type structure for $a$ with respect to $\boldsymbol{\Delta} =\{ \Delta_s,\Delta_x,\Delta \}$. According to this structure, if the policy take action $a=1$ for state $s=\{g,\Delta_s,y,\Delta_x,\Delta\}$, it would takes the same action at state $s=\{g,\Delta_s,y,\Delta_x,\Delta +K \}$, for all $K\in\{0,1,\dots\}$}.
% \begin{proof}
% We show the switching-type structure $\boldsymbol{\Delta}$ for a $\lambda$-optimal policy in preemption scenario, then extend to the blocking scenario. We first show the value function, $h(s)$, is a non-decreasing function respect to $\boldsymbol{\Delta}$.
% we define $Q^i(s,a)$ as
% $$Q^{i}(s,a)=L(s,a, \lambda) +\sum_{s'\in \mathcal{S}}\mathrm{Pr}(s' \mid s,a)h^{i-1}(s')$$
% The value function is obtained as $h^{i}(s)=\min_{a\in \mathcal{A}}\big[Q^{i}(s,a) - Q^{i}(s^{\mathrm{ref}},a)\big]$. Thus, it is sufficient to show that $Q^i(s,a)$ is a non-decreasing function respect to $\boldsymbol{\Delta}$. We use the mathematical induction to proof the non-decreasing property. According to this method, we need to show that the property holds for the initial step. Without loos of generality, we assume $h^0(s)=0$ for all $s\in\mathcal{S}$. For a general state $s=\{1,\Delta_s,1,\Delta_x,\Delta\}$, $Q^1(s,0)$ is derived as
% \begin{equation}\label{q1a0}
% \begin{array}{ll}
%   &\hspace{-8mm}Q^1(s,0) = \Delta +  \gamma p_0h^0(\{0,*,1,\Delta_s+1,\Delta_x+1\}) \\&\hspace{8mm}+  \gamma (1-p_0)h^0(\{0,*,1,\Delta_s+1,\Delta+1\}) \\&\hspace{8mm}+  (1-\gamma) p_0h^0(\{1,\Delta_s+1,0,*,\Delta_x+1\}) \\&\hspace{8mm}+ (1-\gamma) (1-p_0)h^0(\{1,\Delta_s+1,1,\Delta_x+1,\Delta+1\})\\&\hspace{6mm}
%   = \Delta,
% \end{array}
% \end{equation}
% and $Q^1(s,1)$ is derived as
%  \begin{equation}
% \begin{array}{ll}
%   &\hspace{-8mm}Q^1(s,1) = \Delta + \lambda+ \gamma p_0h^0(\{0,*,1,1,\Delta_x+1\}) \\&\hspace{8mm}+  \gamma (1-p_0)h^0(\{0,*,1,1,\Delta+1\}) \\&\hspace{8mm}+  (1-\gamma) p_0h^0(\{1,1,0,*,\Delta_x+1\}) \\&\hspace{8mm}+ (1-\gamma) (1-p_0)h^0(\{1,1,1,\Delta_x+1,\Delta+1\})\\&\hspace{6mm}
%   = \Delta+\lambda,
% \end{array}
% \end{equation}
% thus, the value iteration function is derived as $h^1(s) = \min_{a\in\mathcal{A}}\{Q^1(s,0),Q^1(s,1)\}-D^1 = \Delta-D^1$, where $D^1=Q^1(s^{\mathrm{ref}})$.
% Now, we derive the same for $Q^2(s,a)$, where $Q^2(s,0)$ is derived as
% \begin{equation}\label{q2a0}
% \begin{array}{ll}
%   &\hspace{-8mm}Q^2(s,0) = \Delta +  \gamma p_0h^1(\{0,*,1,\Delta_s+1,\Delta_x+1\}) \\&\hspace{8mm}+  \gamma (1-p_0)h^1(\{0,*,1,\Delta_s+1,\Delta+1\}) \\&\hspace{8mm}+  (1-\gamma) p_0h^1(\{1,\Delta_s+1,0,*,\Delta_x+1\}) \\&\hspace{8mm}+ (1-\gamma) (1-p_0)h^1(\{1,\Delta_s+1,1,\Delta_x+1,\Delta+1\})\\&\hspace{6mm}
%   = \Delta + \gamma p_0 (\Delta_x+1-D^1) + \gamma (1-p_0) (\Delta+1-D^1)\\&\hspace{8mm}+ (1-\gamma) p_0 (\Delta_x+1-D^1) + (1-\gamma) (1-p_0) (\Delta+1-D^1),
% \end{array}
% \end{equation}
% %According to \eqref{q1a0} and \eqref{q2a0}, $Q^i(s,0)$ for initial iterations, i.e., $i=0,1,2$ is non-decreasing respect to $\boldsymbol{\Delta}$.
%  %Now, we derive $Q^1(s,1)$ and $Q^2(s,1)$ as follows: 
% and $Q^2(s,1)$ is derived as
% \begin{equation}\label{q2a1}
% \begin{array}{ll}
%   &\hspace{-8mm}Q^2(s,1) = \Delta +\lambda+  \gamma p_0h^1(\{0,*,1,1,\Delta_x+1\}) \\&\hspace{8mm}+  \gamma (1-p_0)h^1(\{0,*,1,1,\Delta+1\}) \\&\hspace{8mm}+  (1-\gamma) p_0h^1(\{1,1,0,*,\Delta_x+1\}) \\&\hspace{8mm}+ (1-\gamma) (1-p_0)h^1(\{1,1,1,\Delta_x+1,\Delta+1\})\\&\hspace{6mm}
%   =  \Delta+\lambda + \gamma p_0 (\Delta_x+1-D^1) + \gamma (1-p_0) (\Delta+1-D^1)\\&\hspace{8mm}+ (1-\gamma) p_0 (\Delta_x+1-D^1) + (1-\gamma) (1-p_0) (\Delta+1-D^1).
% \end{array}
% \end{equation}
% According to \eqref{q1a0}-\eqref{q2a1}, $Q^i(s,a)$ for initial iterations, i.e., $i=0,1,2$ and all actions is non-decreasing respect to $\boldsymbol{\Delta}$.
% Therefore, the first requirement of induction method hold. Now, we should show, if the non-decreasing property hold for $h^i(s)$, it would hold for $h^{i+1}(s)$. Firstly, we derive $Q^{i+1}(s,a)$ for all actions, $Q^{i+1}(s,0)$ is given as
% \begin{equation}\label{qi+1a0}
% \begin{array}{ll}
%   &\hspace{-8mm}Q^{i+1}(s,0) = \Delta +  \gamma p_0h^i(\{0,*,1,\Delta_s+1,\Delta_x+1\}) \\&\hspace{8mm}+  \gamma (1-p_0)h^i(\{0,*,1,\Delta_s+1,\Delta+1\}) \\&\hspace{8mm}+  (1-\gamma) p_0h^i(\{1,\Delta_s+1,0,*,\Delta_x+1\}) \\&\hspace{8mm}+ (1-\gamma) (1-p_0)h^i1(\{1,\Delta_s+1,1,\Delta_x+1,\Delta+1\}).
% \end{array}
% \end{equation}
% The equation in \eqref{qi+1a0} is a summation of five terms. If we increase $\Delta$ to $\delta+1$, the first term increases as has direction relation with $\Delta$. In addition, third and fifth terms increases or remains unchanged as $h^i$ is a non-decreasing function on the fifth element of the state. The same logic could be applied for other terms of $\boldsymbol{\Delta}$. Now, we derive $Q^{i+1}(s,1)$ given as
% \begin{equation}\label{qi+1a1}
% \begin{array}{ll}
%   &\hspace{-8mm}Q^{i+1}(s,1) = \Delta +  \lambda+  \gamma p_0h^i(\{0,*,1,1,\Delta_x+1\}) \\&\hspace{8mm}+  \gamma (1-p_0)h^i(\{0,*,1,1,\Delta+1\}) \\&\hspace{8mm}+  (1-\gamma) p_0h^i(\{1,1,0,*,\Delta_x+1\}) \\&\hspace{8mm}+ (1-\gamma) (1-p_0)h^i(\{1,1,1,\Delta_x+1,\Delta+1\}).
% \end{array}
% \end{equation}
% With the same logic that mentioned for the $Q^{i+1}(s,0)$, $Q^{i+1}(s,1)$ is also non-decreasing respect to $\boldsymbol{\Delta}$. The same logic for the blocking scenario is true.

% Now, we show the switching type property of the $\lambda$-optimal policy for two scenarios and the states $s_1=\{0,*,0,*,\Delta\}$, $s_2=\{0,*,1,\Delta_x,\Delta\}$, $s_3=\{1,\Delta_s,0,*,\Delta\}$, and $s_4=\{1,\Delta_s,1,\Delta_x,\Delta\}$. Now, we should show that if an optimal
% policy takes action $a=1$ at state $s$, it would take the same action when the age of one of the packets is increased and other elements of the state remain the same. Thus, according to optimal policy expression in \eqref{qopt} and $Q(s,a)$, the following inequality holds
% \begin{equation}\label{inq}
%     \begin{array}{ll}
%          Q(s,1)\leq Q(s,0).%\rightarrow \mathbb{E}\{h(s')\mid s,a=1\}\leq \mathbb{E}\{h(s')\mid s,a=0\}.
%     \end{array}
% \end{equation}
% \textbf{Blocking scenario and $\boldsymbol s_1$}:
% In the following we compute $Q(s_1,1)$ and $Q(s_1,0)$.
% \begin{equation}\label{q+ba1}
% \begin{array}{ll}
%   &\hspace{-8mm}Q(s_1,1) = \Delta +  \lambda+  \gamma h(\{0,*,1,1,\Delta+1\}) \\&\hspace{8mm}+  (1-\gamma) h(\{1,1,0,*,\Delta_+1\}).
% \end{array}
% \end{equation}
% \begin{equation}\label{q+ba0}
% \begin{array}{ll}
%   &\hspace{-8mm}Q(s_1,0) = \Delta+ h(\{0,*,0,*,\Delta+1\}).
% \end{array}
% \end{equation}
% \end{proof}
